Fine-grained Qualitative Spatial Reasoning about Point Positions

The ability to persist in the spacial environment is, not only in the robotic context, an essential feature. Positional knowledge is one of the most important aspects of space and a number of methods to represent these information have been developed in the in the research area of spatial cognition. The basic qualitative spatial representation and reasoning techniques are presented in this thesis and several calculi are briefly reviewed. Features and applications of qualitative calculi are summarized. A new calculus for representing and reasoning about qualitative spatial orientation and distances is being designed. It supports an arbitrary level of granularity over ternary relations of points. Ways of improving the complexity of the composition are shown and an implementation of the calculus demonstrates its capabilities. Existing qualitative spatial calculi of positional information are compared to the new approach and possibilities for future research are outlined.

==> chapters/FSPPimpl.tex <==
% FSPP Diplomarbeit
% Sören Schwertfeger
%
% FSPP implementation
%
% Version 1.0
% Status 	: dann schreib mal!
% Datum		: 8.11.04
%
% FSPPimpl.tex
%

\chapter{FSPP impelementation}


==> chapters/FSPPtest.tex <==
% FSPP Diplomarbeit
% Sören Schwertfeger
%
% FSPPTest
%
% Version 1.0
% Status 	: dann schreib mal!
% Datum		: 8.11.04
%
% FSPPtest.tex
%



==> chapters/vorwort.tex <==
%
% Diplomarbeit mit Latex
% ===========================================================================
% This is part of the book "Diplomarbeit mit LaTeX".
% Copyright (c) 2002 Tobias Erbsland
% See the file main.tex for copying conditions.
%

\chapter{Einleitung}

\section{Motivation}
\label{sec:motivation}

\begin{quote}
"<Es gibt Alternativen zu WYSIWYG\footnote{What You See Is What You Get} Textverarbeitungen">.
\end{quote}

Während einer Diplomarbeit steht man (oft) unter einem starken Zeitdruck. Einen grossen Teil der Zeit, welche du zur Verfügung hast, brauchst du um die Dokumentation zu deiner Arbeit zu schreiben. Viele Studenten begehen den Fehler, dass sie sich keine Gedanken darüber machen, welches die geeignetste Anwendung für ein solch meist umfangreiches Dokument ist. So verschwenden sie einen grossen Teil der Zeit mit ärgerlichen Programmabstürzen, falschen Seitennummerierungen und unerklärlichen Effekten die sich nicht beheben lassen\footnote{Ich beziehe mich in diesen Ausführungen auf Programme wie z.\,B. Microsoft Word. Selbsverständlich gibt es sehr gute WYSIWYG Programme. Es existieren auch sehr gute WYSIWYG Erweiterungen und Editoren welche {\rmfamily\LaTeX} Code direkt grafisch darstellen.}.

Meistens beginnen die Probleme ab einer bestimmten Größe des Dokuments, aber dann ist es oft zu spät um die Anwendung zu wechseln.

Ich möchte dir daher einen einfachen Weg aufzeigen, wie du deine Diplomarbeit oder die Dokumentation dazu mit {\rmfamily\LaTeX} erstellen kannst. Dabei beschreibe ich detailiert den Weg von der Installation einer {\rmfamily\LaTeX}-Distribution unter Windows bis zum ersten lauffähigen Dokument. Weiter beschreibt dieses Dokument häufig benötigte Formatierungen und Themen welche im Zusammenhang einer Diplomarbeit wichtig sind.

\section{Vorschläge und Ergänzungen}

Ich schreibe dieses Dokument in der Hoffnung das es nützlich ist. Daher freue ich mich natürlich über Fehlerberichtigungen und Ergänzungen welche in das Konzept dieses Dokuments passen.

Bevor du Fehler meldest oder oder Vorschläge machst, solltest du kontrollieren ob du die neuste Version dieses Dokuments hast. Die aktuelle Version dieses Dokuments findest du immer unter der folgenden URL:

\href{http://www.dml.drzoom.ch/}{\textbf{http://www.dml.drzoom.ch/}}

\section{Dank}

Folgende Personen haben mich beim Schreiben von diesem Dokument unterstützt. Ich danke Ihnen für Korrekturen, Verbesserungen und Kritik. Daduch ist diese Anleitung wesentlich lesenswerter geworden. 

\begin{itemize}
	\item Christian Faulhammer
	\item Thomas Holenstein
	\item David Kastrup
	\item Markus Kohm
	\item Christian Kuwer
	\item Thomas Ratajczak
	\item Mark Trettin
\end{itemize}

\section{Ausstehende und durchgeführte Änderungen an diesem Dokument}

In Anhang \ref{sec:aendeungen} befindet sich eine Liste welche die Änderungen zwischen den verschiedenen Versionen dieses Dokuments aufzeigt. Daneben findest du eine Liste mit ausstehenden Fragen und Änderungen im Anhang \ref{sec:ausstehendes}.

%
% EOF
%


